Assessing the Emergent Symbolic Reasoning Abilities of Llama Large Language Models

Large Language Models (LLMs) achieve impressive performance in a wide range of tasks, even if they are often trained with the only objective of chatting fluently with users. Among other skills, LLMs show emergent abilities in mathematical reasoning benchmarks, which can be elicited with appropriate prompting methods. In this work, we systematically investigate the capabilities and limitations of popular open-source LLMs on different symbolic reasoning tasks. We evaluate three models of the Llama 2 family on two datasets that require solving mathematical formulas of varying degrees of difficulty. We test a generalist LLM (Llama 2 Chat) as well as two fine-tuned versions of Llama 2 (MAmmoTH and MetaMath) specifically designed to tackle mathematical problems. We observe that both increasing the scale of the model and fine-tuning it on relevant tasks lead to significant performance gains. Furthermore, using fine-grained evaluation measures, we find that such performance gains are mostly observed with mathematical formulas of low complexity, which nevertheless often remain challenging even for the largest fine-tuned models.

==> tables/prompts.tex <==
\begin{tabular}{|p{2cm}|p{4.3cm}|p{5.1cm}|}
        \hline
        \textbf{Model name} & \textbf{Example prompt ListOps} & \textbf{Example prompt Arithmetic} \\
        \hline
        Llama2 & Solve the following arithmetic expression: \texttt{((86+51)+(-74-35))}. Take the modulo 100 of intermediate values, i.e. keep the last two digits of the number with the sign. Give the final answer stating `The final answer is: \texttt{<NUMBER>}'. & \texttt{MIN}, \texttt{MAX} and \texttt{SM} are operators on lists of single-digit integers which have the semantics of minimum, maximum and sum modulo 10, respectively. Solve the following expression involving these operators: \texttt{MAX(3, 9, 1)}. Give the final answer stating 'The final answer is: \texttt{<NUMBER>}'. \\
        \hline
        MAmmoTH & Below is an instruction that describes a task. Write a response that appropriately completes the request.\newline\newline Instruction: Solve the following arithmetic expression: \texttt{((86+51)+(-74-35))}. Take the modulo 100 of intermediate values, i.e. keep the last two digits of the number with the sign.\newline\newline Response: & Below is an instruction that describes a task. Write a response that appropriately completes the request. \newline\newline Instruction: \texttt{MIN}, \texttt{MAX} and \texttt{SM} are operators on lists of single-digit integers which have the semantics of minimum, maximum and sum modulo 10, respectively. Solve the following expression involving these operators: \texttt{MAX(3, 9, 1)}. \newline\newline Response: \\
        \hline
        MetaMath & Below is an instruction that describes a task. Write a response that appropriately completes the request.\newline\newline Instruction: Solve the following arithmetic expression: \texttt{((86+51)+(-74-35))}. Take the modulo 100 of intermediate values, i.e. keep the last two digits of the number with the sign. Give the final answer stating 'The final answer is: \texttt{<NUMBER>}'.\newline\newline Response: Let's think step by step. & Below is an instruction that describes a task. Write a response that appropriately completes the request. \newline\newline Instruction: \texttt{MIN}, \texttt{MAX} and \texttt{SM} are operators on lists of single-digit integers which have the semantics of minimum, maximum and sum modulo 10, respectively. Solve the following expression involving these operators: \texttt{MAX(3, 9, 1)}. Give the final answer stating 'The final answer is: \texttt{<NUMBER>}'. \newline\newline Response: Let's think step by step. \\
        \hline
\end{tabular}
